Structure and statistical organization of the stationary state of the Oslo model

In most driven-dissipative sandpile models, the dynamics of the system reaches a critical stationary state. This state displays organization features such as a power-law avalanche spectrum and hyperuniformity, but these features often emerge without a clear path from the microscopic evolution rules. Only in a few cases is there an available description of the stationary state, in other sandpile models the question is open. In this article, we present our result on the stationary state of the Oslo model, a driven-dissipative sandpile model with intrinsic randomness. In order to do so, we use different representations of the system configurations and of the dynamical process. Moving back and forth between these representations allows to identify invariant quantities for each configurations. Moreover, we obtain the detailed statistical description of the stationary state by considering all paths leading to a given configuration at once, and by summing their contributions under the constraint specified by the invariants. As a result, we find that the configurations of the stationary state are structured into a small number of equivalence classes, and that their statistical weights are related to the counting of colored diagrams respecting a small set of rules.

==> macros.tex <==
%Macros package nomencl
\renewcommand{\nomname}{Nomenclature}
\makeatletter
\newif\if@printfigref
\newif\if@printnoteref
\newif\if@printtableref
\def\nomfigref#1{\if@printfigref\figdeclaration{#1}\fi\ignorespaces}
\def\nomtableref#1{\if@printtableref\tbaledeclaration{#1}\fi\ignorespaces}
\def\nomnoteref#1{\if@printnoteref\notedeclaration{#1}\fi\ignorespaces}
\def\nomrefeqpage{\@printeqreftrue\@printfigreffalse\@printnotereffalse\@printpagereftrue}
\def\nomreffigpage{\@printfigreftrue\@printeqreffalse\@printnotereffalse\@printpagereftrue}
\def\nomreftablepage{\@printtablereftrue\@printeqreffalse\@printnotereffalse\@printpagereftrue}
\def\nomrefnotepage{\@printfigreffalse\@printeqreffalse\@printnotereftrue\@printpagereftrue}
\def\nomrefeq{\@printeqreftrue\@printfigreffalse\@printnotereffalse}
\def\nomrefpage{\@printpagereftrue\@printfigreffalse\@printnotereffalse}
\def\figdeclaration#1{, see Figure\nobreakspace#1}
\def\notedeclaration#1{, see note\nobreakspace#1}
\def\tabledeclaration#1{, see Table\nobreakspace#1}
\def\@@@nomenclature[#1]#2#3{%
 \def\@tempa{#2}\def\@tempb{#3}%
 \protected@write\@nomenclaturefile{}%
  {\string\nomenclatureentry{#1\nom@verb\@tempa @[{\nom@verb\@tempa}]%
      \begingroup\nom@verb\@tempb
      \protect\nomeqref{\theequation}%
      \protect\nomfigref{\thefigure}%
      \protect\nomnoteref{\thefootnote}%
        |nompageref}{\thepage}}%
 \endgroup
 \@esphack}
\makeatother
\def\nomenclhead#1{%
  %\vskip 2em\item[\hbox to \textwidth{\centerline{\bfseries\large{#1}}}]} 
  \vskip 2em\item[\hskip 2 cm\large{#1}]\ \\} 
\renewcommand{\nomgroup}[1]{
  \ifthenelse{\equal{#1}{W}}{\nomenclhead{Words}}{
  \ifthenelse{\equal{#1}{A}}{\nomenclhead{Latin notations}}{
  \ifthenelse{\equal{#1}{G}}{\nomenclhead{Greek notations}}{
  \ifthenelse{\equal{#1}{S}}{\nomenclhead{Other}}{
  \ifthenelse{\equal{#1}{Z}}{\nomenclhead{Diagrammatic notations}}{}}
}}}}
\renewcommand\nomentryend{.}
\makenomenclature

% Notations used along the paper
% C
\newcommand\coloring{\mathrm{Col}}
\newcommand\colorleg{\mathrm{Col}\sp{\star}}
\newcommand\compset[1][]{\mathrm{Comp}\sb{#1}}
\newcommand\stable{\mathcal{C}}
% E
\newcommand\evol{\mathsf{E}}
\newcommand\evolacc{\mathsf{E}_{\textrm{acc}}}
\newcommand\evolution{\mathcal{E}}
\newcommand\evolutionacceptable{\mathcal{E}_{\textrm{acc}}}
% F
\newcommand\setconstraints[1][]{\mathcal{F}\sb{#1}}
% G
\newcommand\general{\mathcal{G}}
% N
\newcommand\N{\mathbf{N}}
% P
\newcommand\final[1][]{\mathcal{P}\sb{#1}}
% R
\newcommand\recur{\mathcal{R}}
\newcommand\recurnat{\mathcal{R}\sb{\textrm{nat}}}
% S
\newcommand\SI{SI}
\newcommand\SRI{SRI}
\newcommand\STI{STI}
\newcommand\stat{\mathcal{S}}
 % T 
\newcommand\domain[1][]{\mathcal{T}\sb{#1}}
\newcommand\toppling[1][]{\mathsf{T}\sb{#1}} 
% W
\newcommand\avalanche{\mathsf{W}}
% Z
\newcommand\zc{z\sb{\text{c}}}
% EPSILON
\newcommand\eps[2][]{\epsilon\sb{#1}\sp{#2}}
% GAMMA
\newcommand\gam[2][]{\mathsf\gamma\sb{#1}\sp{#2}}
% PSI
\newcommand\stst{\psi}

% Decorations
\newcommand\lift[1]{{#1}^\uparrow}
\newcommand\liftnat[1]{\lift{\nat{#1}}}
\newcommand\nat[1]{\tilde{#1}}
\newcommand\instr[2][black]{\ensuremath{\color{#1}\textbf{#2}}}
\newcommand\instrsub[3][black]{\ensuremath{\color{#1}\textbf{#2}\sb{#3}}}

% https://tex.stackexchange.com/questions/1874/how-to-make-a-larger-dot
\DeclareRobustCommand\w[1]{%
  \accentset{\smash{\mbox{\LARGE\bfseries .}}}{#1}}
\DeclareRobustCommand\ww[1]{%
  \accentset{\smash{\mbox{\LARGE\bfseries .\hspace{-0.25ex}.}}}{#1}}
\DeclareRobustCommand\www[1]{%
  \accentset{\smash{\mbox{\LARGE\bfseries .\hspace{-0.35ex}.\hspace{-0.35ex}.}}}{#1}}
\DeclareRobustCommand\Aw[1]{%
  \accentset{\smash{\mbox{\color{purple}\LARGE\bfseries .}}}{#1}}
\DeclareRobustCommand\Aww[1]{%
  \accentset{\smash{\mbox{\LARGE\bfseries .\color{purple}\hspace{-0.25ex}.}}}{#1}}
  
\newcommand\A[1]{{\color{purple}{a}_{#1}}}

\newcommand*\ws[2][1]{%
  \accentset{\smash{\mbox{\itshape\scriptsize #1}}}{#2}}
\newcommand*\Aws[2][1]{%
  \accentset{\smash{\mbox{\color{purple}\itshape\scriptsize #1}}}{#2}}

% Maths
\newcommand\intrange[2]{\llbracket#1,\,#2\rrbracket}

% Configurations
% g
\newcommand\gcfg[1]{\left[{#1}\right]}
% z
\newcommand\zcfg[1]{\left|{#1}\right\rangle}
\newcommand\zgst[2]{\mathchoice%
  {\left|\begin{array}{c}{#1}\\{#2}\end{array}\right\rangle} 
  {\left|\begin{smallmatrix}{#1}\\{#2}\end{smallmatrix}\right\rangle} 
  {\left|\begin{smallmatrix}{#1}\\{#2}\end{smallmatrix}\right\rangle} 
  {\left|\begin{smallmatrix}{#1}\\{#2}\end{smallmatrix}\right\rangle} 
}

%Setup to generically perform operation on each leaf of a tree
\forestset{
  every leaf node/.style={
    if n children=0{#1}{}
  },
  every tree node/.style={
    if n children=0{}{#1}
  },
}

\newcommand\xaxis[2]{
    \draw[->,line width=0.3mm,arrows = {-Stealth}] (0,0) -- (#1,0) node[right]{$x$};
    %\foreach \i in {#2} \draw [line width=0.5mm](\i*0.5+0.25,0)--(\i*0.5+0.25,.1);
    \foreach \i in {#2}
    \node[below] at (\i*0.5-0.25,0){$\i$};
}
\newcommand\yaxis[3]{
    \draw[->,line width=0.3mm,arrows = {-Stealth}] (0,0) -- (0,#1) node[right]{#3};
    \foreach \i in {#2} 
      \node[left] at (0,\i*0.5-0.25) {$\i$};
}

%  Command for generic drawing 
\newcommand\reprzg[2][]{
  \coordinate (ZG) at (0,0); 
  \pgfmathsetmacro{\nbsites}{0} 
  \foreach[count=\x] \z/\w in {#2} {
    \pgfmathsetmacro{\tmp}{\nbsites+1}
    \global\let\nbsites\tmp
    \ifnum\z>0\foreach \y in {1,...,\z}
    { \fill[#1] (ZG) ++(\x*0.5-0.25,\y*0.25) circle (0.1); }
    \fi
    \ifnum\w>0\foreach \y in {1,...,\w}
    { \fill[#1, opacity=0.5] (ZG) ++(\x*0.5-0.25, \z*0.25+\y*0.25) circle (0.11); }
    \fi
  }
  \draw[step=0.5] (ZG) ++(0,-0.125) grid ++(0.5*\nbsites,0.25);
}

%  Command for generic drawing constraints
\newcommand\reprcstr[3][]{
  \coordinate (ZG) at (0,0); 
  \pgfmathsetmacro{\nbsites}{0} 
  \foreach[count=\x] \z/\w in {#2} {
    \pgfmathsetmacro{\tmp}{\nbsites+1}
    \global\let\nbsites\tmp
    \ifnum\z>0\foreach \y in {1,...,\z}
    { \fill[#1, opacity=0] (ZG) ++(\x*0.5-0.25,\y*0.25) circle (0.1); }
    \fi
    \ifnum\w>0\foreach \y in {1,...,\w}
    { \fill[#1] (ZG) ++(\x*0.5-0.25, \z*0.5+\y*0.25) circle (#3); }
    \fi
  }
}

%  Command for generic drawing 
\newcommand\reprhg[2][]{
  \coordinate (HG) at (0,0);
  \pgfmathsetmacro{\nbsites}{0} 
  \foreach[count=\x] \h/\w in {#2} {
    \pgfmathsetmacro{\tmp}{\nbsites+1}
    \global\let\nbsites\tmp
    \ifnum\h>0\foreach \y in {1,...,\h}{
      \draw[#1] (HG) ++(\x*0.5-0.5,\y*0.5-0.5) rectangle ++(0.5,0.5);
    }\fi
    \ifnum\w>0\foreach \y in {1,...,\w}{
      \fill[#1, opacity=0.5] (HG) ++(\x*0.5-0.25,\h*0.5+\y*0.5-0.25) circle (0.11);
    }\fi
  }
  \draw (HG) -- ++(0.5*\nbsites,0);
}

%  Command for generic drawing 
\newcommand\reprgg[2][]{
  \coordinate (GG) at (0,0);
  \pgfmathsetmacro{\nbsites}{0} 
  \foreach[count=\x] \z/\w in {#2} {
    \pgfmathsetmacro{\tmp}{\nbsites+1}
    \global\let\nbsites\tmp
    \ifnum\z>0\foreach \y in {1,...,\z}
      { \draw[#1] (GG) ++(\x*0.5-0.45,\y*0.5-0.45) rectangle ++(0.4,0.4); }
    \fi
    \ifnum\w>0\foreach \y in {1,...,\w}{
      \fill[#1,draw=black,opacity=0.5] (GG) 
            ++(\x*0.5-0.45,\z*0.5+\y*0.5-0.45) rectangle ++(0.4,0.4);
            %\fill[#1,opacity=0.5] (\x*0.5-0.25,\z*0.5 + \y*0.5 -0.25) circle (0.18);
    }
    \fi
  }
  %\draw[step=0.5] (GG) grid ++(0.5*\nbsites,0);
  \draw[step=0.5] (GG) grid ++(0.5*\nbsites,0.1);
}

\newcommand\reprz[3]{
  \coordinate (ZR) at (0,0);
  \pgfmathsetmacro{\nbsites}{0} 
  \foreach[count=\x] \z in {#1} {
  \pgfmathsetmacro{\tmp}{\nbsites+1}
  \global\let\nbsites\tmp
  \ifnum\z>0
    \foreach \y in {1,...,\z}{
      \fill[#3] (ZR) ++(\x*#2-#2*0.5,\y*#2*0.5) circle (#2*0.2); 
    }\fi
  }
  \draw[step=#2] (ZR) ++(0,-#2*0.25) grid ++(#2*\nbsites,#2*0.5);
}

\newcommand\reprh[3]{
  \coordinate (HR) at (0,0);
  \pgfmathsetmacro{\nbsites}{0} 
  \foreach[count=\x] \z in {#1} {
  \pgfmathsetmacro{\tmp}{\nbsites+1}
  \global\let\nbsites\tmp
  \ifnum\z>0
  \foreach \y in {1,...,\z}{
   \draw[#3] (HR) ++(\x*#2-#2,\y*#2-#2) rectangle ++(#2,#2); 
  }\fi
  }
\draw[step=#2] (HR) ++(0,-#2*0.25) grid ++(#2*\nbsites,#2*0.5);
}

\newcommand\reprg[3]{
  \coordinate (GR) at (0,0);
  \pgfmathsetmacro{\nbsites}{0} 
  \foreach[count=\x] \z in {#1} {
  \pgfmathsetmacro{\tmp}{\nbsites+1}
  \global\let\nbsites\tmp
  \ifnum\z>0
    \foreach \y in {1,...,\z}{
      \draw[#3] (GR) ++(\x*#2-#2*0.9,\y*#2-0.9*#2) rectangle ++(#2*0.8,#2*0.8); 
      \node[white] at (\x*#2-0.9*#2,\y*#2) {.};
    }\fi
  }
  \draw[step=#2] (0,0) grid (#2*\nbsites,#2*0.25);
}

\newcommand\topplingarrow[3]{
% x position toppling %height arrow %size arrow (radius) %color arrow 
  \foreach[count=\x] \h in {#1} {
    \ifthenelse{\h>0} {
      \draw[->,color=#3] (\x*0.5-0.25,#2) 
                         arc[radius=0.25, start angle=180, end angle=0];
    } {}
  }
}

\newcommand\topplingleftarrow[3]{%x position toppling %height arrow %size arrow (radius) %color arrow 
  \foreach[count=\x] \h in {#1} {
    \ifthenelse{\h>0}
    {\draw[->,color=#3] (\x*0.5-0.25,#2) arc[radius=0.25, start angle=0, end angle=180];}
    {}
  }
}

%Mathematical notations
\newtheorem{definition}{Definition}[section]
\newtheorem{theorem}[definition]{Theorem}
\newtheorem{corollary}{Corollary}[definition]
\newtheorem{lemma}[definition]{Lemma}
\newtheorem{prop}[definition]{Proposition}
\newtheorem{remark}{Remark}[section]
\newtheorem{conjecture}{Conjecture}[section]

\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmax}{argmax}
\newcommand\Z[1][]{\mathbf{Z}\sp{#1}}
%----------------------------------------------------------------------------------------
%	BIBLIOGRAPHY
%----------------------------------------------------------------------------------------

% Filename of the bibliography
\addbibresource{bibliography.bib} 

